NTIRE 2025 Challenge on Short-form UGC Video Quality Assessment and Enhancement: Methods and Results

This paper presents a review for the NTIRE 2025 Challenge on Short-form UGC Video Quality Assessment and Enhancement. The challenge comprises two tracks: (i) Efficient Video Quality Assessment (KVQ), and (ii) Diffusion-based Image Super-Resolution (KwaiSR). Track 1 aims to advance the development of lightweight and efficient video quality assessment (VQA) models, with an emphasis on eliminating reliance on model ensembles, redundant weights, and other computationally expensive components in the previous IQA/VQA competitions. Track 2 introduces a new short-form UGC dataset tailored for single image super-resolution, i.e., the KwaiSR dataset. It consists of 1,800 synthetically generated S-UGC image pairs and 1,900 real-world S-UGC images, which are split into training, validation, and test sets using a ratio of 8:1:1. The primary objective of the challenge is to drive research that benefits the user experience of short-form UGC platforms such as Kwai and TikTok. This challenge attracted 266 participants and received 18 valid final submissions with corresponding fact sheets, significantly contributing to the progress of short-form UGC VQA and image superresolution. The project is publicly available at https://github.com/lixinustc/KVQE- ChallengeCVPR-NTIRE2025.

==> sec/4_Teams_and_Methods.tex <==
\section{Teams and Methods of Track 1}
\label{sec:teams_and_methods_1}
The details of all 9 teams and their methods can be found in the \textbf{Supplementary}. 
% \textcolor{red}{Need to be checked and revised by team SharpMind. Please substitute the Fig. 1 with the original image in the figures. Thanks.}

\subsection{SharpMind}
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/SharpMind.png} % 替换为你的图像文件名
  % 图注
  % \caption{The student network in the second stage. }
  \caption{The overall framework of Team SharpMind. }
  \label{fig:SharpMind}
\end{figure}
% \subsubsection{Method Description}
This team employs several powerful backbone networks to extract features associated with the human vision system. Subsequently, they train a comprehensive video quality assessment model, which is then utilized as a teacher model to label a series of User-Generated Content (UGC) video datasets. Leveraging these labeled datasets, they train a lightweight student network. As a result, the small-scale model can also effectively discern video quality.

Their method consists of two stages: (i) In the first stage, a comprehensive teacher network is trained by extracting video features through a series of powerful backbone networks. In the second stage, a series of closed-source UGC videos are annotated with pseudo labels by the teacher network and then used to train a lightweight model. They introduce the two stages in detail below.

In the first stage, they extract keyframes of the video following the RQ-VQA \cite{RQ-VQA} strategy. Then, they extract features of these keyframes from three aspects: spatial, temporal, and spatiotemporal. Specifically, they extract the motion features of the video through SlowFast, FAST-VQA features, LIQE features, and DeQA \cite{DeQA} features. In addition, considering that UGC videos are uploaded by ordinary users, these videos often exhibit eye-related characteristics such as edge masking that need to be taken into account. Therefore, they refer to HVS-5M \cite{HVS-5M} to further extract edge and content features of the keyframes. Based on the above features, they fully retain the information of all dimensions of the video. To better preserve the learning of quality-aware features by some learnable parameters, they incorporate an additional Swin-B network. By integrating these features, they train a powerful teacher network. Specifically, they concatenate all of the above features and obtain the final video score through two MLP layers. Due to the integration of a series of features, the teacher model trained in the first stage possesses strong capabilities in identifying the quality of UGC videos. They then use it to annotate a large set of closed-source UGC videos (nearly 30{,}000), providing pseudo labels for training the student model in the second stage.

In the second stage, they utilize a lightweight student network to fit the labels annotated by the teacher network. Their expectation is that the student model can acquire the proficiency to discriminate the quality of UGC videos. Specifically, they first use the keyframe extraction method of RQ-VQA to convert all videos into frame-level representations. Subsequently, the score of each frame is annotated as the score of the corresponding video. After that, they randomly crop a patch with a resolution of $224\times224$ from these frames and feed it into a Swin-T network. Considering the importance of multi-scale features in quality assessment tasks, they obtain the features of each layer of the Swin-T and concatenate them together. Finally, they compute the video quality score through two fully connected layers. 

% \subsubsection{Training details}
\noindent \textbf{Training details} They employ several powerful backbone networks to extract features associated with the human vision system. Subsequently, they train a comprehensive video quality assessment model, which is utilized as a teacher model to label a series of closed-source User-Generated Content (UGC) video datasets. Leveraging these labeled datasets, they train a lightweight network. As a result, the small-scale model can also effectively discern video quality. Differentiable SRCC and PLCC losses are adopted in both training phases.

In the first stage, the keyframes are randomly and centrally cropped to a resolution of $384\times384$ and then fed into the Swin-B network. The Adam optimizer with an initial learning rate of $1 \times 10^{-5}$ and a batch size of 6 is used to train the proposed teacher model on one A100 GPU.

In the second stage, the Adam optimizer with an initial learning rate of $1 \times 10^{-3}$ and a batch size of 64 is used to train the proposed student model on one A100 GPU.




\subsection{ZQE}
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/ZQE.png} % 替换为你的图像文件名
  % 图注
  % \caption{The architecture of the proposed method.}
  \caption{The overall framework of Team ZQE. }
  \label{fig:ZQE}
\end{figure}


This team extracts semantic, local texture, and global features from videos through three branches, aggregates them via an attention mechanism, and finally maps them into a quality score. Their model is a hybrid model built upon and improved from DOVER \cite{DOVER} and KSVQE \cite{KSVQE}.

First, they pretrain DOVER on the KVQ dataset, freeze the aesthetic branch weights, and discard the original VQA head. They then integrate the attention-based fusion modules proposed in KSVQE between each stage of the technical branch. Next, through extensive ablation experiments, they select VideoMamba-middle \cite{VideoMamba} as their video semantic extractor, as it is an effective and lightweight video/image classification model. Specifically, they freeze VideoMamba's pretrained weights obtained from ImageNet-1k \cite{ImageNet} and insert eight trainable MLP modules into the backbone (one after every four SSM layers) to facilitate fine-tuning for the VQA task. Additionally, to address the issue of large irrelevant regions commonly found in short-form videos, they not only incorporate the quality-aware region selection module from KSVQE but also introduce a novel slicing preprocessing step. Specifically, they horizontally divide each video into multiple slices of equal height, compute the texture density of each slice using the Laplacian operator, and discard slices whose texture density falls below a threshold determined empirically from their experiments on the KVQ dataset. This preprocessing approach significantly improves the performance of their model.

Their model is pretrained end-to-end on a combined dataset consisting of the KVQ training set and their private UGC dataset. Finally, they fine-tune the best-performing pretrained model (selected based on validation performance on the KVQ validation set) using the KVQ training set to obtain the optimal model.

% \subsubsection{Training details}
\noindent \textbf{Training details} They first pretrain DOVER on the KVQ dataset and freeze the weights of the aesthetic branch. The technical branch is initialized using the official weights of KSVQE. The model is pretrained end-to-end on a mixed dataset containing the KVQ training set and their private UGC dataset, and is then fine-tuned on the KVQ training set. All training stages are evaluated on the KVQ validation set.

% \subsubsection{Testing details}
\noindent \textbf{Testing details} The test video is directly fed into the model for inference to obtain the predicted quality score. It is important to note that under the current Torch/CUDA version, they observe that multithreading and cuBLAS may introduce non-determinism in the results. Specifically, the output score may vary from the 7th or 8th decimal place onward with some probability. They ensure that no randomness is artificially introduced at any stage of inference. This does not affect the overall score on the Codalab leaderboard (rounded to 4 decimal places: 0.9158).


\subsection{ZX-AIE-Vector}
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/ZX-AIE-Vector.PNG} % 替换为你的图像文件名
  % 图注
  % \caption{Illustration of Mamba-in-Mamba-Out VQA framework. }
  \caption{The overall framework of Team ZX-AIE-Vector. }
  \label{fig:ZX-AIE-Vector}
\end{figure}
% \subsubsection{Method Description}
This team proposes a lightweight and efficient VQA framework to address the limitations of high computational cost and suboptimal performance in many existing Video Quality Assessment methods. The total computational complexity of their framework is constrained to approximately 100 GFLOPS. Specifically, their approach adopts a widely used dual-stream architecture that separately extracts spatial-temporal and temporal features. For spatial-temporal modeling, they design two lightweight modules: a low-resolution branch to capture coarse global context, and a high-resolution branch to extract fine-grained local details, which are subsequently fused. Meanwhile, a lightweight SlowFast \cite{slowfast} module is employed to extract multi-scale temporal features. 

To further enhance the model’s representation capability, they introduce a Multi-Scale Parallel Mamba (MSPM) layer. This module leverages the global modeling ability and linear complexity of Mamba \cite{mamba} to perform deep feature extraction, improving long-range dependency modeling. Finally, spatial-temporal and temporal features are fused to form a comprehensive video representation. Experiments on the S-UGC competition dataset KVQ \cite{KSVQE} demonstrate that their method achieves competitive performance while maintaining high efficiency, validating the effectiveness of the proposed lightweight dual-stream architecture and the MSPM module.

% \subsubsection{Training details}
\noindent \textbf{Training details} The training pipeline consists of three main stages: pretraining, pseudo-labeling, and two-phase fine-tuning. They first pretrain their lightweight model on the large-scale LSVQ dataset \cite{LSVQ} for 10 epochs to learn generalizable video representations, strictly following the original training-validation split. 

Next, they fine-tune a large-scale model on the KVQ dataset \cite{KSVQE} (merging the official training and validation sets), and use it to generate pseudo-labels for the test set. These pseudo-labels are then merged with the original KVQ training and validation data to construct an augmented dataset.

They conduct the first-phase fine-tuning of their lightweight model using this augmented set via 10-fold cross-validation, training each fold for 30 epochs. The average prediction across all folds is used as a refined pseudo-label for each test sample. In the second-phase fine-tuning, they use the full KVQ training and validation sets along with the refined pseudo-labeled test data to retrain their lightweight model for an additional 30 epochs. This two-stage fine-tuning strategy enables them to fully exploit the unlabeled test data and improve generalization.

They implement their method using PyTorch and train it on 8 NVIDIA V100 GPUs. The Adam optimizer is used with an initial learning rate of $3\times10^{-5}$, combined with a Cosine Annealing learning rate scheduler that gradually decreases the learning rate to a minimum of $1\times10^{-6}$. The entire training process takes approximately 9 hours.

% \subsubsection{Testing details}
\noindent \textbf{Testing details} During testing, they evaluate their final lightweight model on the KVQ test set. For each video, they uniformly sample 8 frames, consistent with the training pipeline. The input resolution during testing is kept the same as in training to ensure consistency in feature extraction. The model directly predicts a quality score for each video. To ensure reproducibility, they fix the random seed to 8 during all testing procedures.


\subsection{ECNU-SJTU VQA Team}
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/ECNU-SJTU VQA Team.png} % 替换为你的图像文件名
  % 图注
  % \caption{The framework of the proposed model. }
  \caption{The overall framework of Team ECNU-SJTU. }
  \label{fig:ECNU-SJTU VQA Team}
\end{figure}
% \subsubsection{Method Description}
This team proposes an efficient video quality assessment (VQA) model named E-VQA~\cite{ntire2025EVQA}, designed to achieve high performance while maintaining low computational complexity. Inspired by previous successful efforts in developing efficient VQA models such as SimpleVQA \cite{SimpleVQA}, FAST-VQA \cite{Fast-vqa}, and MinimalisticVQA \cite{MinimalisticVQA}, they empirically explore a combination of best practices from these models along with techniques from other efficient deep neural networks (DNNs) to develop E-VQA. By combining task-specific and general optimizations, their method balances accuracy and efficiency for practical deployment.

They begin with the lightweight MinimalisticVQA VIII model \cite{MinimalisticVQA}, replacing its backbone from Swin Transformer-Base to Swin Transformer-Tiny (Swin-T) \cite{swin}, and evaluate the optimal frame count and resolution under the competition’s computational constraint of 120 GFLOPs. Next, they incrementally integrate motion features (extracted via X3D \cite{X3d}) and fragment frame features (extracted using 2D/3D FAST-VQA variants \cite{Fast-vqa}) into the baseline to assess performance gains.
Their experiments reveal that a dual Swin-T architecture with shared weights achieves optimal results. One branch aligns with MinimalisticVQA VIII, processing frames resized to $384\times384$, while the other employs a 2D FAST-VQA variant operating on fragment frames composed of $12 \times 12$ image patches with a resolution of $32 \times 32$. For feature extraction, they uniformly sample 4 frames from 8-second video clips.

To enhance generalization, they adopt an offline knowledge distillation strategy using RQ-VQA \cite{RQ-VQA}—the winning solution of the NTIRE 2024 VQA Challenge—as the teacher model. They curate a pretraining dataset of 52,000 videos, consisting of 40,000 web-sourced videos and 12,000 synthetically compressed samples. Specifically, they generate 2,000 originals from the web-sourced videos and compress them using H.264 at 6 levels \cite{KSVQE}. RQ-VQA is used to generate pseudo-labels for all videos. Finally, they pretrain E-VQA on this dataset using fidelity loss \cite{fidelity} and RMSE loss, and fine-tune it on the KVQ training set using PLCC loss. The source code and dataset will be publicly released to ensure reproducibility. The final test score achieved is 0.91083.

The \textbf{Training Details} and \textbf{Testing Details} of this team can be found in the \textbf{Supplementary}. 

% \subsubsection{Training details}



==> sec/5_Teams_and_Methods.tex <==
\section{Teams and Methods of Track 2}
\label{sec:teams_and_methods_2}
The details of all 8 teams and their methods can be found in the \textbf{Supplementary}. 
\subsection{TACO\_SR}
% Done!
This team develops a two-stage super-resolution method, including an image super-resolution phase and an image fusion phase, as shown in Figure~\ref{fig:TACO_SR}. Their method consists of three key components designed to generate a high-quality image: (1) PiSASR~\cite{sun2024pixelPiSASR}, (2) Detail Extractor, and (3) NAFusion (Inspired by NAFSSR~\cite{chu2022nafssr}). They optimize the NAFusion module based on KwaiSR dataset, while keeping pre-trained PiSASR fixed.

In the first phase, they develop their method based on PiSASR~\cite{sun2024pixelPiSASR}. They generate candidate images uder two different settings: (1) $\lambda_{\text{pix}} = 1.0, \lambda_{\text{sem}} = 0.0$: This configuration prioritizes high fidelity, producing an image denoted as $I_{\text{psnr}}$; and (2) $\lambda_{\text{pix}} = 1.0, \lambda_{\text{sem}} = 1.0$: This setting enhances perceptual quality, resulting in an image referred to as $I_{\text{per}}$. They observe that $I_{\text{psnr}}$ achieves superior fidelity (PSNR, SSIM) but lacks perceptual quality (NIQE, MANIQA, CLIPIQA). Conversely, $I_{\text{per}}$ excels in perceptual quality but exhibits lower fidelity. They take advantage of $I_{\text{psnr}}$ and $I_{\text{per}}$ by an image fusion model. Specifically, they first combine $I_{\text{psnr}}$ and $I_{\text{per}}$ to $I_{\text{init}}$ with Detail Extractor: use high pass filter to extract high frequency component from $I_{\text{per}}$ and add to $I_{\text{psnr}}$. 

In the second phase, they construct NAFusion using $I_{\text{psnr}}$, $I_{\text{per}}$, and $I_{\text{init}}$. Inspired by NAFSSR~\cite{chu2022nafssr}, they design the NAFusion module with NAFBlock and SCAM. Finally, they add $I_{\text{init}}$ to the output of the main branch of NAFusion to generate $I_{\text{HQ}}$.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/TACO_SR.png}
    \caption{The overall framework of Team PiNAFusion-SR.}
    \label{fig:TACO_SR}
\end{figure}

\noindent \textbf{Training Details}
First, they generate $I_{\text{psnr}}$ and $I_{\text{per}}$ from low-quality images in the provided training dataset using PiSASR under different settings. ($I_{\text{psnr}}$: $\lambda_{\text{pix}} = 1.0, \lambda_{\text{sem}} = 0.0$, $I_{\text{per}}$: $\lambda_{\text{pix}} = 1.0, \lambda_{\text{sem}} = 1.0$). Then, they crop image patches from $I_{\text{psnr}}$, $I_{\text{per}}$ and $I_{\text{GT}}$ with $512 \times 512$ resolution (Overlap is set to 128). They train NAFusion $f$ using data triplet $(I_{\text{psnr}}, I_{\text{per}}, I_{\text{GT}})$ with a loss function $L_{\text{total}}$:
\begin{equation}
L_{\text{total}} = \lambda_1 L_{\text{pix}} + \lambda_2 L_{\text{ssim}} + \lambda_3 L_{\text{lpips}},
\end{equation}
where
\begin{align*}
L_{\text{pix}}\  &= L_1(f(I_{\text{psnr}}, I_{\text{per}}), I_{\text{GT}}) \text{ is L1 loss}, \\
L_{\text{ssim}} &= L_{\text{SSIM}}(f(I_{\text{psnr}}, I_{\text{per}}), I_{\text{GT}}) \text{ is SSIM loss}, \\
L_{\text{lpips}} &= L_{\text{LPIPS}}(f(I_{\text{psnr}}, I_{\text{per}}), I_{\text{GT}}) \text{ is LPIPS loss}.
\end{align*}

They set the batch size and the learning rate to 8 and $1e^{- 5}$. They train NAFusion for 5 epochs, with $\lambda_1 = 10.0, \lambda_2 = 0.5, \lambda_3 = 1.0$.

\noindent \textbf{Testing Details}
They set the scale factor to 4 and 1 when running inference with PiNAFusion-SR on images from the ``synthetic'' and ``wild'' subfolders in the validation and test datasets. The scaling strategy is determined based on the resolution of the input image. Specifically, if the larger dimension (height or width) of the input image is below 500 pixels, they apply a scale factor of 4. Otherwise, they use a scale factor of 1. They perform inference on both the validation and test datasets using the same settings.

\subsection{RealismDiff}
% Done!
This team proposes a two-stage diffusion-based image super-resolution method consisting of the PreCleaner (a lightweight CNN) and SUPIR~\cite{yu2024scalingsupir}. Specifically, as shown in Figure.~\ref{fig:realismdiff}, they construct a dynamic pipeline to assign different processing paths according to the image quality assessment. For images with weak degradation, they use a light restoration module (or resize function) to maintain the high-frequency information and fewer step diffusion, while using more extensive settings (larger CNN and diffusion model with more steps and higher CFG) for heavily distorted images. Besides, they collect a training dataset of high-resolution images from DIV2K~\cite{agustsson2017ntireDIV2K}, Flicker2K~\cite{lim2017enhancedFlik2K}, FFHQ~\cite{kazemi2014oneFFHQ}, and Laion5B~\cite{schuhmann2022Laion5B}.

\noindent \textbf{Training Details}
They train the proposed method using 8 A100 GPUs and adopt the AdamW optimizer with default parameters. During training, they crop images into patches of 512$\times$512 pixels and set the batch size as 32. They first pre-train the PreCleaner for 1000 iterations with an initial learning rate of $5\times e^{-5}$. They then fine-tune the entire pipeline in an end-to-end manner for 40,000 iterations. During the fine-tuning stage, the learning rate for the ControlNet is initialized as $5\times e^{-6}$. The learning rates are updated using the Cosine
Annealing scheme.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/RealismDiff.png}
    \caption{The framework proposed by Team RealismDiff.}
    \label{fig:realismdiff}
\end{figure}


\subsection{SRlab}
% Done!
As shown in Figure~\ref{fig:SRlab}, the method of this team~\cite{wang2025enhancedtopthree} is based on the diffusion framework. They employ a VAE to encode the input low-quality images and obtain their corresponding latent representations. These latents are then processed by a Denoising U-Net, which iteratively refines them through multiple denoising steps. To ensure the generated images maintain high fidelity with the low-resolution (LR) inputs, they incorporate the ControlNet architecture, which allows for precise control over the generation process. Furthermore, recognizing that the official synthetic and wild test sets exhibit varying degrees of degradation and require different super-resolution scaling factors, they enhance their approach by utilizing the Segment Anything Model 2~\cite{ravi2024sam} (SAM2). SAM2 is employed to extract rich semantic embeddings from these images, providing additional contextual information that aids in the denoising process. The extracted latents, enriched with semantic embeddings, are subsequently fed into the Denoising U-Net for T steps of iterative refinement. During training, they optimize their model by minimizing the denoising objective:
\begin{equation}
    \mathcal{L} = \mathbb{E}_{X_0,X_{lr},t,c,c_{\text{sem}},\epsilon} \left\|\epsilon - \epsilon_{\theta}(X_t, X_{lr}, t, c, c_{\text{sem}})\right\|^2,
\end{equation}
where $X_{lr}$ represents the low-resolution (LR) latent, $c$ denotes the tag prompt, and $c_{\text{sem}}$ is the semantic embedding. The noise estimation network $\epsilon_{\theta}$ is responsible for predicting the noise $\epsilon \sim \mathcal{N}(0, I)$.
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/SRlab.png}
    \caption{Overall Pipeline of the solution of Team SRlab.}
    \label{fig:SRlab}
\end{figure}

\noindent \textbf{Training Details}
To enhance the model’s performance in short-form UGC scenarios, they constructed a new training dataset by combining the synthetic training set provided by the competition with the LSDIR dataset~\cite{li2023lsdir}. First, they processed the high-resolution images from the LSDIR training set by applying a $4\times$ downsampling and degradation with a 50\% probability for each of two degradation modes to simulate the image degradation scenarios in the synthetic and wild datasets, respectively. Second, they refined the synthetic training set (1440 pairs of gt and lr images) by cropping and overlapping its high-resolution (1080×1920) images to generate $512\times 512$ sub-images, which served as ground truth (GT) images. These GT images were then 4× downsampled and degraded to create the corresponding low-resolution images. Finally, they merged the processed LSDIR training set with the synthetic training set to form the final dataset for training.

They trained the model on a synthesized 512$\times$512 dataset for 90,000 steps using an Nvidia RTX 3090 GPU and the Adam optimizer with a learning rate of $5\times e^{-5}$. The original Stable Diffusion parameters were frozen, and only the ControlNet component and semantic embedding transformer module were trained. The implementation was built on PyTorch, with mixed precision training (FP16) and gradient accumulation to optimize efficiency.

\noindent \textbf{Testing Details}
During the testing phase, they analyzed the impact of three key parameters: ``start point'', ``guidance scale(gs)'', and positive/negative prompts on the experimental results.

First, they evaluated the model’s performance on both the synthetic and wild datasets by setting ``start point'' to either ``noise'' or ``lr'' while keeping ``gs = 5.5'' without adding additional prompts. Next, with ``gs = 5.5'', they introduced positive prompts (``ultra-detailed'', ``ultra-realistic'') and negative prompts (``distorted'', ``deformed'') separately, comparing the model’s overall performance in each case. Finally, they examined the model’s final scores across different ``gs'' values. Based on the results, they selected the best-performing parameter combination for the final test settings.

\subsection{SYSU-FVL-Team}
% Done!
This team develops the framework based on diffusion. They leverage the diffusion model to predict the residual between LQ latent feature and HQ latent feature rather than directly predict HQ latent feature itself. Such a residual learning formulation helps the model focus on learning the desired high-frequency information from the HQ latent features, and it can also accelerate the convergence of the model training process~\cite{he2016deep}. The predicted HQ latent feature will be decoded into high-quality images by the decoder. In order to adjust the preference between pixel and visual semantics, they add a dual LoRA module controlling the pixel-wise and semantic-wise quality based on the pretrained diffusion model SD21, similar to PiSASR~\cite{sun2024pixelPiSASR}.

Following PiSASR, they introduce a pair of pixel and semantic guidance factors, denoted by $\lambda_{\text{pix}}$ and $\lambda_{\text{sem}}$, to control the SR results as follows:
\begin{equation}
\epsilon_\theta(z_L) = \lambda_{\text{pix}}\epsilon_{\theta_{\text{pix}}}(z_L) + \lambda_{\text{sem}}(\epsilon_{\theta_{\text{PiS A}}}(z_L) - \epsilon_{\theta_{\text{pix}}}(z_L)),
\end{equation}
where $\epsilon_{\theta_{\text{pix}}}(z_L)$ is the output with only pixel-level LoRA, and $\epsilon_{\theta_{\text{PiS A}}}(z_L)$ is the output with both pixel and semantic level enhancement. When processing synthetic images, $\lambda_{\text{pix}}$ and $\lambda_{\text{sem}}$ are set as 1.0 and 0.5 to process wild images, separately.

The \textbf{Training Details} of this team can be found in the \textbf{Supplementary}





